TopoMan: Global Network Visibility in the Presence of Middleboxes (A Graybox Approach)

Software Defined Networks (SDN) provide vital benefits to network administrators by offering global visibility and network-wide control over the switching infrastructure of the network. It is rather much difficult to obtain the same benefits in the presence of middleboxes (MBs), due to (i) lack of a proper topology discovery mechanism in environments with a mix of forwarding devices and middleboxes. (ii) lack of generic APIs to abstract and gain control on these rigid and heterogeneous third-party middleboxes (iii) lack of a generic network infrastructure framework to monitor and verify any specific device or path connectivity status in the network. These limitations make automation of network operations such as, network-wide monitoring, policy enforcement and rule-placement much difficult to handle. Hence, there is a greater urge even from middlebox vendors, to better handle the control and visibility aspects of the network in presence of middleboxes. In this paper, we propose a Unified network infrastructure framework for gaining global network visibility, by discovering the network topology in the presence of middleboxes, along with a framework to support the end-to-end path connectivity verification, independent of SDN. We have also addressed security aspects and provided necessary APIs to support our framework.

==> acknowledgement.tex <==
We thank Ayon Chakrobarthy for his valuable feedback. 

==> assumptions.tex <==
The middleboxes are initially expected to be configured with infrastructure forwarding/routing rules to forward the probe messages. The topology discovery mechanism showcased in this paper is limited to devices with management capabilities.

==> implementtest.tex <==
%\vspace{1mm}\\
\textbf{Implementation.} The main functional components are implemented in c \& python. The MB Agent in each of middlebox runs a UDP based transparent proxy module and uses iptables(Netfilter) rules for probe traffic redirection.  The \textit{Probe Tracking \& Control} module in the middlebox handles the post routing functions using the iptables and ip rules and a python based monitor module is developed to handle the outgoing probe messages. The \textit{Topology Manager} is a simple python based network manager designed to handle the messages(REST) from both SDN(floodlight) and MB Controller. The MB Controller is the python based controller interfaced to the middleboxes and the topology manager. \vspace{1mm}\\
\textbf{Test Environment.} 
\textbf{Our topology discovery mechanism is tested considering Cisco's small and medium scale enterprise network deployment scenarios \& setups described here\cite{Smallscaleenterprisedesignprofile,Mediumscaledesignprofile}.}

\textbf{The test environment includes mix of different topologies specific to enterprise networks such as inline, offline, tree and star. Middlebox functions are built with few third-aprty middleboxes and remaining PC based systems integrated with open-sources based middlebox functions such as openvpn\cite{OPENVPN}, IPSec vpn OpenSwan\cite{OPENSWAN} squid\cite{SQUID}, Netfilter (Linux based Network Firewall)\cite{netfilter}, vconfig\cite{VCONFIG}, openvswitch\cite{OPENVSWITCH} for specially testing topology discovery with VPN, web-proxy, firewall and VLAN functions.}

\textbf{The payload security is tested by integrating Nacl(salt)\cite{NACL} with the MB Agent and Topology Manager, which is considered as light weight module with better latency parameters when compared with openssl\cite{FASTERNACL}. Our implementation used iptables and ip rules to handle the probe messages, these rules introduces negligible latency to the general traffic. }
\vspace{1mm}\\
\textbf{Compatibility.} The code changes that we introduced in middleboxes are purely infrastructure(routing) changes, with no impact on actual middlebox functions. As most of the third-party middlebox vendors such as Cisco\cite{Cisco}, Juniper\cite{Juniper}, Barracuda Networks\cite{Barracuda} and \textbf{so on}, supports the port(transport) based routing functionality in their middleboxes, it is much easier to integrate both the probe-based functions in their devices.

\textbf{Assumptions.} The middleboxes are initially expected to be configured with infrastructure forwarding/routing rules to forward the probe messages.

